A Constant-Factor Approximation for Continuous Dynamic Time Warping in 2D

Continuous Dynamic Time Warping (CDTW) is a robust similarity measure for polygonal curves that has recently found a variety of applications. Despite its practical use, not much is known about the algorithmic complexity of computing it in 2D, especially when one requires either an exact solution or strong approximation guarantees. We fill this gap by introducing a $5$-approximation algorithm with running time $O(n^5)$ under the 1-norm. This is the first constant-factor approximation for 2D CDTW with polynomial running time. We extend our algorithm to all polygonal norms on $\mathbb{R}^2$, which we subsequently use in order to achieve a $(5+\varepsilon)$-approximation with time complexity $O(n^5 / \varepsilon^{1/2})$ for CDTW in 2D under any fixed norm. The latter result in particular includes the usual Euclidean 2-norm.

==> preamble.tex <==
\usepackage[T1]{fontenc}
\usepackage{microtype}

\makeatletter
    \DeclareRobustCommand\small{%
        \@setfontsize\small\@xpt\@xiipt
        \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
        \abovedisplayshortskip \z@ \@plus3\p@
        \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
        \def\@listi{\leftmargin\leftmargini
            \topsep 6\p@ \@plus2\p@ \@minus2\p@
            \parsep 3\p@ \@plus2\p@ \@minus\p@
            \itemsep \parsep}%
        \belowdisplayskip \abovedisplayskip
    }
    \DeclareRobustCommand\footnotesize{%
        \@setfontsize\footnotesize\@ixpt{11}%
        \abovedisplayskip 8\p@ \@plus2\p@ \@minus4\p@
        \abovedisplayshortskip \z@ \@plus\p@
        \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
        \def\@listi{\leftmargin\leftmargini
            \topsep 4\p@ \@plus2\p@ \@minus2\p@
            \parsep 2\p@ \@plus\p@ \@minus\p@
            \itemsep \parsep}%
        \belowdisplayskip \abovedisplayskip
    }
\makeatother


\usepackage{float,caption,subcaption}
\setlength{\intextsep}{8pt plus 1pt minus 1pt}
\captionsetup{
    font=small,
    labelfont=bf,
    labelsep=period,
    justification=centering,
}
\subcaptionsetup{
    font=footnotesize,
    justification=centering,
}


\usepackage{enumerate}
\newenvironment*{alphaenumerate}%
    {\begin{enumerate}[\upshape(a)]}%
    {\end{enumerate}}
\makeatletter
    \newenvironment*{alphaenumerate*}{%
        \let\orig@listi\@listi%
        \def\@listi{\orig@listi\topsep=0pt}%
        \begin{alphaenumerate}
    }{
        \end{alphaenumerate}%
        \def\@listi{\orig@listi}%
    }
\makeatother


\usepackage{hyperref,xurl,xpatch}
\hypersetup{hidelinks,hypertexnames=false,bookmarksdepth=2}
\makeatletter
    \xpatchcmd{\@spbegintheorem}{\hskip}{\MakeLinkTarget{\@currentcounter}\hskip}{}{}
    \xpatchcmd{\@spopargbegintheorem}{\hskip}{\MakeLinkTarget{\@currentcounter}\hskip}{}{}
\makeatother

\newcommand*{\autoappref}[1]{\hyperref[#1]{Appendix~\ref*{#1}}}
\newcommand*{\propagatecosts}{\hyperref[alg:propagate-costs]{\textsc{PropagateCosts}}}
\newcommand*{\propagatefromadj}{\hyperref[alg:propagate-from-adj]{\textsc{PropagateFromAdjoining}}}
\newcommand*{\propagatefromopp}{\hyperref[alg:propagate-from-opp]{\textsc{PropagateFromOpposing}}}

\usepackage[UKenglish]{babel}
\addto\extrasUKenglish{%
    \renewcommand*{\sectionautorefname}{Section}%
    \renewcommand*{\subsectionautorefname}{Section}%
    \providecommand*{\algorithmautorefname}{Algorithm}%
}


\usepackage{amssymb,mathtools,ifthen}
\mathtoolsset{centercolon}

\newcommand*{\ds}{\:\mathrm{d}s}
\newcommand*{\dt}{\:\mathrm{d}t}
\newcommand*{\trianglerho}{\;\!\triangleright}
\newcommand*{\rhoinput}[1][\mathcal{A}]{\rho_{#1}^{\trianglerho}}
\newcommand*{\rhooutput}[1][\mathcal{B}]{\rho^{#1}_{\trianglerho}}

\newcommand*{\tnorm}[1][]{%
    \ifthenelse{\equal{#1}{}}%
        {\mbox{$\| \cdot \|$}}%
        {\mbox{$\| \cdot \|_{#1}$}}%
}
\newcommand*{\settheoremcounter}[1]{%
    \setcounterref{theorem}{#1}%
    \addtocounter{theorem}{-1}%
}

\newcommand*{\kernedN}[1][\mkern-2mu]{\ensuremath{\mkern2mu\mathcal{N}#1}}
\newcommand*{\kernedE}[1][\mkern-1mu]{\ensuremath{\mkern1mu\mathcal{E}#1}}
\newcommand*{\kernedS}[1][\mkern-1mu]{\ensuremath{\mkern1mu\mathcal{S}#1}}
\newcommand*{\kernedW}[1][\mkern-1mu]{\ensuremath{\mathcal{W}#1}}

\DeclareMathSymbol{\Gamma}{\mathalpha}{operators}{"00}
\DeclareMathSymbol{\Delta}{\mathalpha}{operators}{"01}
\DeclareMathSymbol{\Theta}{\mathalpha}{operators}{"02}
\DeclareMathSymbol{\Lambda}{\mathalpha}{operators}{"03}
\DeclareMathSymbol{\Xi}{\mathalpha}{operators}{"04}
\DeclareMathSymbol{\Pi}{\mathalpha}{operators}{"05}
\DeclareMathSymbol{\Sigma}{\mathalpha}{operators}{"06}
\DeclareMathSymbol{\Upsilon}{\mathalpha}{operators}{"07}
\DeclareMathSymbol{\Phi}{\mathalpha}{operators}{"08}
\DeclareMathSymbol{\Psi}{\mathalpha}{operators}{"09}
\DeclareMathSymbol{\Omega}{\mathalpha}{operators}{"0A}


\usepackage{algorithm,algorithmicx,xspace}
\algrenewcommand{\algorithmicindent}{.5\parindent}
\algrenewcommand{\alglinenumber}[1]{{\footnotesize#1.}}
\algrenewcommand{\algorithmiccomment}[1]{%
    \hfill%
    {%
        \ttfamily\color{black!60!white}%
        \smash{//~#1}%
    }%
    \rule{0pt}{0pt}%
}

\algblockdefx{For}{EndFor}[1]{\algFor #1\ \algDo}{}
\algblockdefx{Foreach}{EndForeach}[1]{\algForeach #1\ \algDo}{}
\algblockdefx{Procedure}{EndProcedure}[2]{\algProcedure \textsc{#1}(#2)}{}
\algtext*{EndFor}
\algtext*{EndForeach}
\algtext*{EndProcedure}

\algnewcommand{\iIf}[1]{\State \algIf #1\ \algThen}
\algnewcommand{\iFor}[1]{\State \algFor #1\ \algDo}
\algnewcommand{\Return}[1]{\State \algReturn #1}
\algnewcommand{\algkw}[1]{{\ttfamily\bfseries#1}\xspace}

\algnewcommand{\algIf}{\algkw{if}}
\algnewcommand{\algThen}{\algkw{then}}
\algnewcommand{\algFor}{\algkw{for}}
\algnewcommand{\algTo}{\algkw{to}}
\algnewcommand{\algDo}{\algkw{do}}
\algnewcommand{\algForeach}{\algkw{foreach}}
\algnewcommand{\algWith}{\algkw{with}}
\algnewcommand{\algReturn}{\algkw{return}}
\algnewcommand{\algProcedure}{\algkw{procedure}}

